PanoDR: Spherical Panorama Diminished Reality for Indoor Scenes

The rising availability of commercial $360^\circ$ cameras that democratize indoor scanning, has increased the interest for novel applications, such as interior space re-design. Diminished Reality (DR) fulfills the requirement of such applications, to remove existing objects in the scene, essentially translating this to a counterfactual inpainting task. While recent advances in data-driven inpainting have shown significant progress in generating realistic samples, they are not constrained to produce results with reality mapped structures. To preserve the `reality' in indoor (re-)planning applications, the scene's structure preservation is crucial. To ensure structure-aware counterfactual inpainting, we propose a model that initially predicts the structure of an indoor scene and then uses it to guide the reconstruction of an empty -- background only -- representation of the same scene. We train and compare against other state-of-the-art methods on a version of the Structured3D dataset modified for DR, showing superior results in both quantitative metrics and qualitative results, but more interestingly, our approach exhibits a much faster convergence rate. Code and models are available at https://vcl3d.github.io/PanoDR/ .

==> Layout.tex <==
A core module of our approach is the estimation of the room layout, which later with drive the hallucination of realistic samples. To this end we employ the well established \textbf{UNet} architecture originally proposed in \cite{ronneberger2015u}. The network consists of 4 down-sampling and up-sampling convolutional modules (refer to \ref{fig:networks}) for the detailed architecture. \textbf{EDW THA DWSW KAI KAPOIA DETAILS MALLON GIA TO ARCH ALLA AFOU GINEI TO SXHMA}. The sole purpose of the network is to predict the dense room layout (see fig\ref{data_generation}d) of an masked image. We approach this task as a classification task, where each pixel of the input image can be one of the \textit{ceiling, wall, floor} classes. This network is supervised by the dense room layouts of the dataset (see fig\ref{data_generation}d) with \textit{Cross Entropy loss}. \textbf{+ EQUATION, ALLA DEN KSERW TI ALLO MPOROUME NA POUME EDW}.

==> teaser_figure.tex <==


\begin{figure*}
    \includegraphics[width=\textwidth]{figures/teaser/teaser.png}
    \centering
\end{figure*}
